BehaVerify: Verifying Temporal Logic Specifications for Behavior Trees

Behavior Trees, which originated in video games as a method for controlling NPCs but have since gained traction within the robotics community, are a framework for describing the execution of a task. BehaVerify is a tool that creates a nuXmv model from a py_tree. For composite nodes, which are standardized, this process is automatic and requires no additional user input. A wide variety of leaf nodes are automatically supported and require no additional user input, but customized leaf nodes will require additional user input to be correctly modeled. BehaVerify can provide a template to make this easier. BehaVerify is able to create a nuXmv model with over 100 nodes and nuXmv was able to verify various non-trivial LTL properties on this model, both directly and via counterexample. The model in question features parallel nodes, selector, and sequence nodes. A comparison with models based on BTCompiler indicates that the models created by BehaVerify perform better.

==> Images/build/processed_data/blueROV/elapsed_build.tex <==
\begin{table}
\centering
\caption{blueROV, Time in Seconds to Create .smv}
\label{blueROV_build}
\begin{tabular}{llll}
\toprule
{} & Leaf\_v2 & Total\_v2 & Total\_v3 \\
\midrule
full          &    0.70 &     0.60 &     0.60 \\
small         &    0.60 &     0.60 &     0.60 \\
warnings\_only &    0.60 &     0.60 &     0.60 \\
\bottomrule
\end{tabular}
\end{table}


==> Images/build/processed_data/checklist/elapsed_build.tex <==
\begin{table}
\centering
\caption{checklist, Time in Seconds to Create .smv}
\label{checklist_build}
\begin{tabular}{lllll}
\toprule
{} &   BTC & Leaf\_v2 & Total\_v2 & Total\_v3 \\
\midrule
1  &  0.10 &    0.10 &     0.10 &     0.10 \\
2  &  0.10 &    0.10 &     0.10 &     0.10 \\
3  &  0.10 &    0.10 &     0.10 &     0.10 \\
4  &  0.10 &    0.10 &     0.10 &     0.10 \\
5  &  0.10 &    0.10 &     0.10 &     0.10 \\
6  &  0.10 &    0.10 &     0.10 &     0.10 \\
7  &  0.10 &    0.10 &     0.10 &     0.10 \\
8  &  0.10 &    0.10 &     0.10 &     0.10 \\
9  &  0.10 &    0.10 &     0.10 &     0.10 \\
10 &  0.10 &    0.10 &     0.10 &     0.10 \\
11 &  0.10 &    0.10 &     0.10 &     0.10 \\
12 &  0.10 &    0.10 &     0.10 &     0.10 \\
13 &  0.10 &    0.10 &     0.10 &     0.10 \\
14 &  0.10 &    0.10 &     0.10 &     0.10 \\
15 &  0.10 &    0.10 &     0.10 &     0.10 \\
16 &  0.10 &    0.10 &     0.10 &     0.10 \\
17 &  0.10 &    0.10 &     0.10 &     0.10 \\
18 &  0.10 &    0.10 &     0.10 &     0.10 \\
19 &  0.10 &    0.10 &     0.10 &     0.10 \\
20 &  0.10 &    0.10 &     0.10 &     0.10 \\
21 &  0.10 &    0.10 &     0.10 &     0.10 \\
22 &  0.10 &    0.10 &     0.10 &     0.10 \\
23 &  0.10 &    0.10 &     0.10 &     0.10 \\
24 &  0.10 &    0.10 &     0.10 &     0.10 \\
25 &  0.10 &    0.10 &     0.10 &     0.10 \\
26 &  0.10 &    0.10 &     0.10 &     0.10 \\
27 &  0.10 &    0.10 &     0.10 &     0.10 \\
28 &  0.10 &    0.10 &     0.10 &     0.10 \\
29 &  0.10 &    0.10 &     0.10 &     0.10 \\
30 &  0.10 &    0.10 &     0.10 &     0.10 \\
31 &  0.10 &    0.10 &     0.10 &     0.10 \\
32 &  0.10 &    0.10 &     0.10 &     0.10 \\
33 &  0.10 &    0.10 &     0.10 &     0.10 \\
34 &  0.10 &    0.10 &     0.10 &     0.10 \\
35 &  0.10 &    0.10 &     0.10 &     0.10 \\
36 &  0.10 &    0.10 &     0.10 &     0.10 \\
37 &  0.10 &    0.10 &     0.10 &     0.10 \\
38 &  0.10 &    0.10 &     0.10 &     0.10 \\
39 &  0.10 &    0.10 &     0.10 &     0.10 \\
40 &  0.10 &    0.10 &     0.10 &     0.10 \\
41 &  0.10 &    0.10 &     0.10 &     0.10 \\
42 &  0.10 &    0.10 &     0.10 &     0.10 \\
43 &  0.10 &    0.10 &     0.10 &     0.10 \\
44 &  0.10 &    0.10 &     0.10 &     0.10 \\
45 &  0.10 &    0.10 &     0.10 &     0.10 \\
46 &  0.10 &    0.10 &     0.10 &     0.10 \\
47 &  0.10 &    0.10 &     0.10 &     0.10 \\
48 &  0.10 &    0.10 &     0.10 &     0.10 \\
49 &  0.10 &    0.10 &     0.10 &     0.10 \\
50 &  0.10 &    0.10 &     0.10 &     0.10 \\
\bottomrule
\end{tabular}
\end{table}


==> Images/build/processed_data/parallel-checklist/elapsed_build.tex <==
\begin{table}
\centering
\caption{parallel-checklist, Time in Seconds to Create .smv}
\label{parallel-checklist_build}
\begin{tabular}{lllll}
\toprule
{} &   BTC & Leaf\_v2 & Total\_v2 & Total\_v3 \\
\midrule
1  &  0.10 &    0.10 &     0.10 &     0.10 \\
2  &  0.10 &    0.10 &     0.10 &     0.10 \\
3  &  0.10 &    0.10 &     0.10 &     0.10 \\
4  &  0.10 &    0.10 &     0.10 &     0.10 \\
5  &  0.10 &    0.10 &     0.10 &     0.10 \\
6  &  0.10 &    0.10 &     0.10 &     0.10 \\
7  &  0.10 &    0.10 &     0.10 &     0.10 \\
8  &  0.10 &    0.10 &     0.10 &     0.10 \\
9  &  0.10 &    0.10 &     0.10 &     0.10 \\
10 &  0.10 &    0.10 &     0.10 &     0.10 \\
11 &  0.10 &    0.10 &     0.10 &     0.10 \\
12 &  0.10 &    0.10 &     0.10 &     0.10 \\
13 &  0.10 &    0.10 &     0.10 &     0.10 \\
14 &  0.10 &    0.10 &     0.10 &     0.10 \\
15 &  0.10 &    0.10 &     0.10 &     0.10 \\
16 &  0.10 &    0.10 &     0.10 &     0.10 \\
17 &  0.10 &    0.10 &     0.10 &     0.10 \\
18 &  0.10 &    0.10 &     0.10 &     0.10 \\
19 &  0.10 &    0.10 &     0.10 &     0.10 \\
20 &  0.10 &    0.10 &     0.10 &     0.10 \\
21 &  0.10 &    0.10 &     0.10 &     0.10 \\
22 &  0.10 &    0.10 &     0.10 &     0.10 \\
23 &  0.10 &    0.10 &     0.10 &     0.10 \\
24 &  0.10 &    0.10 &     0.10 &     0.10 \\
25 &  0.10 &    0.10 &     0.10 &     0.10 \\
26 &  0.10 &    0.10 &     0.10 &     0.10 \\
27 &  0.10 &    0.10 &     0.10 &     0.10 \\
28 &  0.10 &    0.10 &     0.10 &     0.10 \\
29 &  0.10 &    0.10 &     0.10 &     0.10 \\
30 &  0.10 &    0.10 &     0.10 &     0.10 \\
31 &  0.10 &    0.10 &     0.10 &     0.10 \\
32 &  0.10 &    0.10 &     0.10 &     0.10 \\
33 &  0.10 &    0.10 &     0.10 &     0.10 \\
34 &  0.10 &    0.10 &     0.10 &     0.10 \\
35 &  0.10 &    0.10 &     0.10 &     0.10 \\
36 &  0.10 &    0.10 &     0.10 &     0.10 \\
37 &  0.10 &    0.10 &     0.10 &     0.10 \\
38 &  0.10 &    0.10 &     0.10 &     0.10 \\
39 &  0.10 &    0.10 &     0.10 &     0.10 \\
40 &  0.10 &    0.10 &     0.10 &     0.10 \\
41 &  0.10 &    0.10 &     0.10 &     0.10 \\
42 &  0.10 &    0.10 &     0.10 &     0.10 \\
43 &  0.10 &    0.10 &     0.10 &     0.10 \\
44 &  0.10 &    0.10 &     0.10 &     0.10 \\
45 &  0.10 &    0.10 &     0.10 &     0.10 \\
46 &  0.10 &    0.10 &     0.10 &     0.10 \\
47 &  0.10 &    0.10 &     0.10 &     0.10 \\
48 &  0.10 &    0.10 &     0.10 &     0.10 \\
49 &  0.10 &    0.10 &     0.10 &     0.10 \\
50 &  0.10 &    0.10 &     0.10 &     0.10 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/build/processed_data/checklist/elapsed_build.tex <==
\begin{table}
\centering
\caption{checklist, Time in Seconds to Create .smv}
\label{checklist_build}
\begin{tabular}{lllll}
\toprule
{} &   BTC & Leaf\_v2 & Total\_v2 & Total\_v3 \\
\midrule
1  &  0.10 &    0.10 &     0.10 &     0.10 \\
2  &  0.10 &    0.10 &     0.10 &     0.10 \\
3  &  0.10 &    0.10 &     0.10 &     0.10 \\
4  &  0.10 &    0.10 &     0.10 &     0.10 \\
5  &  0.10 &    0.10 &     0.10 &     0.10 \\
6  &  0.10 &    0.10 &     0.10 &     0.10 \\
7  &  0.10 &    0.10 &     0.10 &     0.10 \\
8  &  0.10 &    0.10 &     0.10 &     0.10 \\
9  &  0.10 &    0.10 &     0.10 &     0.10 \\
10 &  0.10 &    0.10 &     0.10 &     0.10 \\
11 &  0.10 &    0.10 &     0.10 &     0.10 \\
12 &  0.10 &    0.10 &     0.10 &     0.10 \\
13 &  0.10 &    0.10 &     0.10 &     0.10 \\
14 &  0.10 &    0.10 &     0.10 &     0.10 \\
15 &  0.10 &    0.10 &     0.10 &     0.10 \\
16 &  0.10 &    0.10 &     0.10 &     0.10 \\
17 &  0.10 &    0.10 &     0.10 &     0.10 \\
18 &  0.10 &    0.10 &     0.10 &     0.10 \\
19 &  0.10 &    0.10 &     0.10 &     0.10 \\
20 &  0.10 &    0.10 &     0.10 &     0.10 \\
21 &  0.10 &    0.10 &     0.10 &     0.10 \\
22 &  0.10 &    0.10 &     0.10 &     0.10 \\
23 &  0.10 &    0.10 &     0.10 &     0.10 \\
24 &  0.10 &    0.10 &     0.10 &     0.10 \\
25 &  0.10 &    0.10 &     0.10 &     0.10 \\
26 &  0.10 &    0.10 &     0.10 &     0.10 \\
27 &  0.10 &    0.10 &     0.10 &     0.10 \\
28 &  0.10 &    0.10 &     0.10 &     0.10 \\
29 &  0.10 &    0.10 &     0.10 &     0.10 \\
30 &  0.10 &    0.10 &     0.10 &     0.10 \\
31 &  0.10 &    0.10 &     0.10 &     0.10 \\
32 &  0.10 &    0.10 &     0.10 &     0.10 \\
33 &  0.10 &    0.10 &     0.10 &     0.10 \\
34 &  0.10 &    0.10 &     0.10 &     0.10 \\
35 &  0.10 &    0.10 &     0.10 &     0.10 \\
36 &  0.10 &    0.10 &     0.10 &     0.10 \\
37 &  0.10 &    0.10 &     0.10 &     0.10 \\
38 &  0.10 &    0.10 &     0.10 &     0.10 \\
39 &  0.10 &    0.10 &     0.10 &     0.10 \\
40 &  0.10 &    0.10 &     0.10 &     0.10 \\
41 &  0.10 &    0.10 &     0.10 &     0.10 \\
42 &  0.10 &    0.10 &     0.10 &     0.10 \\
43 &  0.10 &    0.10 &     0.10 &     0.10 \\
44 &  0.10 &    0.10 &     0.10 &     0.10 \\
45 &  0.10 &    0.10 &     0.10 &     0.10 \\
46 &  0.10 &    0.10 &     0.10 &     0.10 \\
47 &  0.10 &    0.10 &     0.10 &     0.10 \\
48 &  0.10 &    0.10 &     0.10 &     0.10 \\
49 &  0.10 &    0.10 &     0.10 &     0.10 \\
50 &  0.10 &    0.10 &     0.10 &     0.10 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/build/processed_data/parallel-checklist/elapsed_build.tex <==
\begin{table}
\centering
\caption{parallel-checklist, Time in Seconds to Create .smv}
\label{parallel-checklist_build}
\begin{tabular}{lllll}
\toprule
{} &   BTC & Leaf\_v2 & Total\_v2 & Total\_v3 \\
\midrule
1  &  0.10 &    0.10 &     0.10 &     0.10 \\
2  &  0.10 &    0.10 &     0.10 &     0.10 \\
3  &  0.10 &    0.10 &     0.10 &     0.10 \\
4  &  0.10 &    0.10 &     0.10 &     0.10 \\
5  &  0.10 &    0.10 &     0.10 &     0.10 \\
6  &  0.10 &    0.10 &     0.10 &     0.10 \\
7  &  0.10 &    0.10 &     0.10 &     0.10 \\
8  &  0.10 &    0.10 &     0.10 &     0.10 \\
9  &  0.10 &    0.10 &     0.10 &     0.10 \\
10 &  0.10 &    0.10 &     0.10 &     0.10 \\
11 &  0.10 &    0.10 &     0.10 &     0.10 \\
12 &  0.10 &    0.10 &     0.10 &     0.10 \\
13 &  0.10 &    0.10 &     0.10 &     0.10 \\
14 &  0.10 &    0.10 &     0.10 &     0.10 \\
15 &  0.10 &    0.10 &     0.10 &     0.10 \\
16 &  0.10 &    0.10 &     0.10 &     0.10 \\
17 &  0.10 &    0.10 &     0.10 &     0.10 \\
18 &  0.10 &    0.10 &     0.10 &     0.10 \\
19 &  0.10 &    0.10 &     0.10 &     0.10 \\
20 &  0.10 &    0.10 &     0.10 &     0.10 \\
21 &  0.10 &    0.10 &     0.10 &     0.10 \\
22 &  0.10 &    0.10 &     0.10 &     0.10 \\
23 &  0.10 &    0.10 &     0.10 &     0.10 \\
24 &  0.10 &    0.10 &     0.10 &     0.10 \\
25 &  0.10 &    0.10 &     0.10 &     0.10 \\
26 &  0.10 &    0.10 &     0.10 &     0.10 \\
27 &  0.10 &    0.10 &     0.10 &     0.10 \\
28 &  0.10 &    0.10 &     0.10 &     0.10 \\
29 &  0.10 &    0.10 &     0.10 &     0.10 \\
30 &  0.10 &    0.10 &     0.10 &     0.10 \\
31 &  0.10 &    0.10 &     0.10 &     0.10 \\
32 &  0.10 &    0.10 &     0.10 &     0.10 \\
33 &  0.10 &    0.10 &     0.10 &     0.10 \\
34 &  0.10 &    0.10 &     0.10 &     0.10 \\
35 &  0.10 &    0.10 &     0.10 &     0.10 \\
36 &  0.10 &    0.10 &     0.10 &     0.10 \\
37 &  0.10 &    0.10 &     0.10 &     0.10 \\
38 &  0.10 &    0.10 &     0.10 &     0.10 \\
39 &  0.10 &    0.10 &     0.10 &     0.10 \\
40 &  0.10 &    0.10 &     0.10 &     0.10 \\
41 &  0.10 &    0.10 &     0.10 &     0.10 \\
42 &  0.10 &    0.10 &     0.10 &     0.10 \\
43 &  0.10 &    0.10 &     0.10 &     0.10 \\
44 &  0.10 &    0.10 &     0.10 &     0.10 \\
45 &  0.10 &    0.10 &     0.10 &     0.10 \\
46 &  0.10 &    0.10 &     0.10 &     0.10 \\
47 &  0.10 &    0.10 &     0.10 &     0.10 \\
48 &  0.10 &    0.10 &     0.10 &     0.10 \\
49 &  0.10 &    0.10 &     0.10 &     0.10 \\
50 &  0.10 &    0.10 &     0.10 &     0.10 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/processed_data/blueROV/diameters.tex <==
\begin{table}
\centering
\caption{blueROV, System Diameter}
\label{blueROV_diam}
\begin{tabular}{llll}
\toprule
{} & Leaf\_v2 & Total\_v2 & Total\_v3 \\
\midrule
w batt &     126 &        4 &        5 \\
w emer &     126 &        4 &        5 \\
w home &     126 &        4 &        5 \\
w obst &     126 &        4 &        5 \\
w sens &     126 &        4 &        5 \\
s batt &     225 &        4 &        4 \\
s emer &     225 &        4 &        4 \\
s home &     225 &        4 &        4 \\
s obst &     225 &        4 &        4 \\
s sens &     225 &        4 &        4 \\
f batt &     330 &        4 &        5 \\
f emer &     330 &        4 &        5 \\
f home &     330 &        4 &        5 \\
f obst &     330 &        4 &        5 \\
f sens &     330 &        4 &        5 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/processed_data/blueROV/elapsed_model.tex <==
\begin{table}
\centering
\caption{blueROV, Time in Seconds to Build Model}
\label{blueROV_model_time}
\begin{tabular}{llll}
\toprule
{} & Leaf\_v2 & Total\_v2 & Total\_v3 \\
\midrule
w batt &    0.04 &     0.02 &     0.02 \\
w emer &    0.05 &     0.02 &     0.02 \\
w home &    0.04 &     0.02 &     0.01 \\
w obst &    0.04 &     0.02 &     0.01 \\
w sens &    0.04 &     0.01 &     0.02 \\
s batt &    0.04 &     0.02 &     0.02 \\
s emer &    0.05 &     0.02 &     0.02 \\
s home &    0.04 &     0.02 &     0.02 \\
s obst &    0.05 &     0.02 &     0.02 \\
s sens &    0.05 &     0.02 &     0.03 \\
f batt &    0.05 &     0.02 &     0.03 \\
f emer &    0.05 &     0.03 &     0.03 \\
f home &    0.05 &     0.03 &     0.02 \\
f obst &    0.06 &     0.02 &     0.03 \\
f sens &    0.04 &     0.03 &     0.01 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/processed_data/blueROV/elapsed_states.tex <==
\begin{table}
\centering
\caption{blueROV, Time in Seconds to Compute Reachability}
\label{blueROV_states_time}
\begin{tabular}{llll}
\toprule
{} & Leaf\_v2 & Total\_v2 & Total\_v3 \\
\midrule
w batt &    0.01 &     0.00 &     0.00 \\
w emer &    0.01 &     0.00 &     0.00 \\
w home &    0.01 &     0.00 &     0.00 \\
w obst &    0.01 &     0.00 &     0.00 \\
w sens &    0.01 &     0.00 &     0.00 \\
s batt &    1.14 &     0.01 &     0.01 \\
s emer &    1.13 &     0.01 &     0.01 \\
s home &    1.17 &     0.01 &     0.01 \\
s obst &    1.13 &     0.01 &     0.01 \\
s sens &    1.12 &     0.01 &     0.01 \\
f batt &    8.24 &     0.08 &     0.10 \\
f emer &    9.08 &     0.08 &     0.09 \\
f home &    8.29 &     0.08 &     0.10 \\
f obst &    8.43 &     0.07 &     0.10 \\
f sens &    8.32 &     0.09 &     0.09 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/processed_data/blueROV/maximum_resident_ltl.tex <==
\begin{table}
\centering
\caption{blueROV, Maximum Resident Size in K to Compute LTL}
\label{blueROV_LTL_size}
\begin{tabular}{llll}
\toprule
{} & Leaf\_v2 & Total\_v2 & Total\_v3 \\
\midrule
w batt &   37898 &    23164 &    22804 \\
w emer &   40210 &    23836 &    23486 \\
w home &   40210 &        - &    23594 \\
w obst &   40744 &    23796 &    23352 \\
w sens &   40766 &    23630 &    23380 \\
s batt &   70052 &    24816 &    25396 \\
s emer &   71900 &    26722 &    26826 \\
s home &   68600 &        - &    27718 \\
s obst &   69392 &    26526 &    26648 \\
s sens &   71504 &    26410 &    26704 \\
f batt &  171048 &    26610 &    27904 \\
f emer &  173424 &    40120 &    39910 \\
f home &  149796 &        - &    43286 \\
f obst &  165900 &    38566 &    41004 \\
f sens &  174216 &    38406 &    41628 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/processed_data/blueROV/reachable_states.tex <==
\begin{table}
\centering
\caption{blueROV, Reachable States}
\label{blueROV_reach}
\begin{tabular}{llll}
\toprule
{} &      Leaf\_v2 &     Total\_v2 &     Total\_v3 \\
\midrule
w batt &  4.44156e+08 &  2.29888e+06 &  5.15687e+06 \\
w emer &  4.44156e+08 &  2.29888e+06 &  5.15687e+06 \\
w home &  4.44156e+08 &  2.29888e+06 &  5.15687e+06 \\
w obst &  4.44156e+08 &  2.29888e+06 &  5.15687e+06 \\
w sens &  4.44156e+08 &  2.29888e+06 &  5.15687e+06 \\
s batt &  5.55901e+11 &  4.14759e+08 &  6.84096e+08 \\
s emer &  5.55901e+11 &  4.14759e+08 &  6.84096e+08 \\
s home &  5.55901e+11 &  4.14759e+08 &  6.84096e+08 \\
s obst &  5.55901e+11 &  4.14759e+08 &  6.84096e+08 \\
s sens &  5.55901e+11 &  4.14759e+08 &  6.84096e+08 \\
f batt &  1.24419e+15 &  6.56377e+11 &  1.12885e+12 \\
f emer &  1.24419e+15 &  6.56377e+11 &  1.12885e+12 \\
f home &  1.24419e+15 &  6.56377e+11 &  1.12885e+12 \\
f obst &  1.24419e+15 &  6.56377e+11 &  1.12885e+12 \\
f sens &  1.24419e+15 &  6.56377e+11 &  1.12885e+12 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/processed_data/blueROV/total_states.tex <==
\begin{table}
\centering
\caption{blueROV, Total States}
\label{blueROV_total}
\begin{tabular}{llll}
\toprule
{} &      Leaf\_v2 &     Total\_v2 &     Total\_v3 \\
\midrule
w batt &  7.10903e+11 &  3.14573e+07 &  3.14573e+07 \\
w emer &  7.10903e+11 &  3.14573e+07 &  3.14573e+07 \\
w home &  7.10903e+11 &  3.14573e+07 &  3.14573e+07 \\
w obst &  7.10903e+11 &  3.14573e+07 &  3.14573e+07 \\
w sens &  7.10903e+11 &  3.14573e+07 &  3.14573e+07 \\
s batt &  7.37064e+18 &  3.26149e+14 &  3.26149e+14 \\
s emer &  7.37064e+18 &  3.26149e+14 &  3.26149e+14 \\
s home &  7.37064e+18 &  3.26149e+14 &  3.26149e+14 \\
s obst &  7.37064e+18 &  3.26149e+14 &  3.26149e+14 \\
s sens &  7.37064e+18 &  3.26149e+14 &  3.26149e+14 \\
f batt &  6.36824e+22 &  2.81793e+18 &  2.81793e+18 \\
f emer &  6.36824e+22 &  2.81793e+18 &  2.81793e+18 \\
f home &  6.36824e+22 &  2.81793e+18 &  2.81793e+18 \\
f obst &  6.36824e+22 &  2.81793e+18 &  2.81793e+18 \\
f sens &  6.36824e+22 &  2.81793e+18 &  2.81793e+18 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/processed_data/checklist/diameters.tex <==
\begin{table}
\centering
\caption{checklist, System Diameter}
\label{checklist_diam}
\begin{tabular}{lllll}
\toprule
{} & BTC & Leaf\_v2 & Total\_v2 & Total\_v3 \\
\midrule
1  &   2 &       3 &        1 &        1 \\
2  &   3 &       4 &        1 &        1 \\
3  &   4 &       5 &        1 &        1 \\
4  &   5 &       6 &        1 &        1 \\
5  &   6 &       7 &        1 &        1 \\
6  &   7 &       8 &        1 &        1 \\
7  &   8 &       9 &        1 &        1 \\
8  &   9 &      10 &        1 &        1 \\
9  &  10 &      11 &        1 &        1 \\
10 &  11 &      12 &        1 &        1 \\
11 &  12 &      13 &        1 &        1 \\
12 &  13 &      14 &        1 &        1 \\
13 &  14 &      15 &        1 &        1 \\
14 &  15 &      16 &        1 &        1 \\
15 &  16 &      17 &        1 &        1 \\
16 &  17 &      18 &        1 &        1 \\
17 &  18 &      19 &        1 &        1 \\
18 &  19 &      20 &        1 &        1 \\
19 &  20 &      21 &        1 &        1 \\
20 &  21 &      22 &        1 &        1 \\
21 &  22 &      23 &        1 &        1 \\
22 &  23 &      24 &        1 &        1 \\
23 &  24 &      25 &        1 &        1 \\
24 &  25 &      26 &        1 &        1 \\
25 &  26 &      27 &        1 &        1 \\
26 &  27 &      28 &        1 &        1 \\
27 &  28 &      29 &        1 &        1 \\
28 &  29 &      30 &        1 &        1 \\
29 &  30 &      31 &        1 &        1 \\
30 &  31 &      32 &        1 &        1 \\
31 &  32 &      33 &        1 &        1 \\
32 &  33 &      34 &        1 &        1 \\
33 &  34 &      35 &        1 &        1 \\
34 &  35 &      36 &        1 &        1 \\
35 &  36 &      37 &        1 &        1 \\
36 &  37 &      38 &        1 &        1 \\
37 &  38 &      39 &        1 &        1 \\
38 &  39 &      40 &        1 &        1 \\
39 &  40 &      41 &        1 &        1 \\
40 &  41 &      42 &        1 &        1 \\
41 &  42 &      43 &        1 &        1 \\
42 &  43 &      44 &        1 &        1 \\
43 &  44 &      45 &        1 &        1 \\
44 &  45 &      46 &        1 &        1 \\
45 &  46 &      47 &        1 &        1 \\
46 &  47 &      48 &        1 &        1 \\
47 &  48 &      49 &        1 &        1 \\
48 &  49 &      50 &        1 &        1 \\
49 &  50 &      51 &        1 &        1 \\
50 &  51 &      52 &        1 &        1 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/processed_data/checklist/elapsed_ltl.tex <==
\begin{table}
\centering
\caption{checklist, Time in Seconds to Compute LTL}
\label{checklist_LTL_time}
\begin{tabular}{lllll}
\toprule
{} &     BTC & Leaf\_v2 & Total\_v2 & Total\_v3 \\
\midrule
1  &    0.00 &    0.00 &     0.00 &     0.00 \\
2  &    0.00 &    0.01 &     0.00 &     0.00 \\
3  &    0.01 &    0.02 &     0.00 &     0.00 \\
4  &    0.02 &    0.03 &     0.01 &     0.01 \\
5  &    0.03 &    0.06 &     0.03 &     0.01 \\
6  &    0.07 &    0.08 &     0.13 &     0.01 \\
7  &    0.07 &    0.12 &     1.02 &     0.03 \\
8  &    0.11 &    0.17 &     8.51 &     0.03 \\
9  &    0.21 &    0.22 &    43.40 &     0.04 \\
10 &    0.43 &    0.28 &        - &     0.06 \\
11 &    0.26 &    0.37 &        - &     0.07 \\
12 &    0.46 &    0.46 &        - &     0.09 \\
13 &    4.56 &    0.56 &        - &     0.09 \\
14 &    1.29 &    0.70 &        - &     0.12 \\
15 &    1.81 &    0.72 &        - &     0.14 \\
16 &    2.02 &    1.01 &        - &     0.18 \\
17 &    2.02 &    1.17 &        - &     0.20 \\
18 &    1.90 &    1.39 &        - &     0.23 \\
19 &   27.06 &    1.65 &        - &     0.27 \\
20 &   17.79 &    1.83 &        - &     0.32 \\
21 &    7.62 &    2.11 &        - &     0.37 \\
22 &   65.53 &    2.39 &        - &     0.41 \\
23 &   11.09 &    2.73 &        - &     0.43 \\
24 &   31.91 &    2.99 &        - &     0.51 \\
25 &   10.30 &    3.36 &        - &     0.60 \\
26 &   27.16 &    3.75 &        - &     0.64 \\
27 &   20.00 &    4.15 &        - &     0.69 \\
28 &   31.83 &    4.47 &        - &     0.80 \\
29 &  155.39 &    5.00 &        - &     0.88 \\
30 &   30.93 &    5.56 &        - &     1.01 \\
31 &  196.04 &    5.97 &        - &     1.10 \\
32 &   49.11 &    6.60 &        - &     1.37 \\
33 &   56.30 &    7.22 &        - &     1.45 \\
34 &   77.28 &    7.99 &        - &     1.66 \\
35 &   83.78 &    8.74 &        - &     1.74 \\
36 &  107.88 &    9.32 &        - &     1.91 \\
37 &  130.80 &   10.23 &        - &     2.09 \\
38 &  127.55 &   11.02 &        - &     2.26 \\
39 &  143.34 &   11.77 &        - &     2.51 \\
40 &  172.81 &   12.84 &        - &     2.64 \\
41 &  157.92 &   13.57 &        - &     2.85 \\
42 &  191.04 &   14.59 &        - &     2.94 \\
43 &  195.57 &   15.66 &        - &     3.18 \\
44 &  215.02 &   16.80 &        - &     3.43 \\
45 &  251.13 &   18.11 &        - &     3.71 \\
46 &       - &   20.17 &        - &     3.94 \\
47 &       - &   19.79 &        - &     3.58 \\
48 &       - &   21.72 &        - &     4.62 \\
49 &       - &   22.19 &        - &     4.82 \\
50 &       - &   23.96 &        - &     5.10 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/processed_data/checklist/elapsed_model.tex <==
\begin{table}
\centering
\caption{checklist, Time in Seconds to Build Model}
\label{checklist_model_time}
\begin{tabular}{lllll}
\toprule
{} &   BTC & Leaf\_v2 & Total\_v2 & Total\_v3 \\
\midrule
1  &  0.00 &    0.00 &     0.00 &     0.00 \\
2  &  0.00 &    0.00 &     0.00 &     0.00 \\
3  &  0.00 &    0.00 &     0.00 &     0.00 \\
4  &  0.00 &    0.01 &     0.00 &     0.00 \\
5  &  0.00 &    0.00 &     0.00 &     0.00 \\
6  &  0.00 &    0.01 &     0.00 &     0.00 \\
7  &  0.00 &    0.00 &     0.00 &     0.00 \\
8  &  0.00 &    0.01 &     0.00 &     0.00 \\
9  &  0.00 &    0.01 &     0.00 &     0.00 \\
10 &  0.01 &    0.01 &     0.00 &     0.00 \\
11 &  0.00 &    0.01 &     0.00 &     0.00 \\
12 &  0.01 &    0.01 &     0.00 &     0.00 \\
13 &  0.01 &    0.01 &     0.00 &     0.00 \\
14 &  0.01 &    0.01 &     0.00 &     0.00 \\
15 &  0.01 &    0.02 &     0.00 &     0.00 \\
16 &  0.01 &    0.02 &     0.00 &     0.00 \\
17 &  0.01 &    0.02 &     0.00 &     0.00 \\
18 &  0.02 &    0.02 &     0.00 &     0.00 \\
19 &  0.02 &    0.03 &     0.00 &     0.00 \\
20 &  0.03 &    0.03 &     0.00 &     0.00 \\
21 &  0.02 &    0.03 &     0.00 &     0.00 \\
22 &  0.02 &    0.03 &     0.01 &     0.01 \\
23 &  0.03 &    0.04 &     0.01 &     0.00 \\
24 &  0.03 &    0.03 &     0.00 &     0.00 \\
25 &  0.03 &    0.04 &     0.01 &     0.00 \\
26 &  0.03 &    0.03 &     0.01 &     0.01 \\
27 &  0.03 &    0.03 &     0.00 &     0.00 \\
28 &  0.04 &    0.04 &     0.00 &     0.01 \\
29 &  0.05 &    0.05 &     0.00 &     0.01 \\
30 &  0.05 &    0.04 &     0.01 &     0.00 \\
31 &  0.07 &    0.05 &     0.00 &     0.01 \\
32 &  0.07 &    0.05 &     0.00 &     0.01 \\
33 &  0.06 &    0.04 &     0.01 &     0.01 \\
34 &  0.07 &    0.04 &     0.01 &     0.01 \\
35 &  0.07 &    0.05 &     0.01 &     0.01 \\
36 &  0.08 &    0.06 &     0.01 &     0.01 \\
37 &  0.09 &    0.06 &     0.01 &     0.01 \\
38 &  0.09 &    0.06 &     0.01 &     0.01 \\
39 &  0.10 &    0.06 &     0.01 &     0.01 \\
40 &  0.09 &    0.06 &     0.01 &     0.01 \\
41 &  0.11 &    0.06 &     0.01 &     0.01 \\
42 &  0.11 &    0.07 &     0.01 &     0.00 \\
43 &  0.11 &    0.07 &     0.01 &     0.01 \\
44 &  0.13 &    0.07 &     0.01 &     0.00 \\
45 &  0.13 &    0.08 &     0.01 &     0.01 \\
46 &  0.13 &    0.07 &     0.01 &     0.01 \\
47 &  0.15 &    0.07 &     0.01 &     0.01 \\
48 &  0.15 &    0.08 &     0.01 &     0.01 \\
49 &  0.17 &    0.08 &     0.01 &     0.01 \\
50 &  0.15 &    0.09 &     0.01 &     0.01 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/processed_data/checklist/elapsed_states.tex <==
\begin{table}
\centering
\caption{checklist, Time in Seconds to Compute Reachability}
\label{checklist_states_time}
\begin{tabular}{lllll}
\toprule
{} &   BTC & Leaf\_v2 & Total\_v2 & Total\_v3 \\
\midrule
1  &  0.00 &    0.00 &     0.00 &     0.00 \\
2  &  0.00 &    0.00 &     0.00 &     0.00 \\
3  &  0.00 &    0.00 &     0.00 &     0.00 \\
4  &  0.00 &    0.00 &     0.00 &     0.00 \\
5  &  0.00 &    0.00 &     0.00 &     0.00 \\
6  &  0.00 &    0.00 &     0.00 &     0.00 \\
7  &  0.00 &    0.00 &     0.00 &     0.00 \\
8  &  0.00 &    0.00 &     0.00 &     0.00 \\
9  &  0.00 &    0.00 &     0.00 &     0.00 \\
10 &  0.01 &    0.00 &     0.00 &     0.00 \\
11 &  0.00 &    0.00 &     0.00 &     0.00 \\
12 &  0.00 &    0.00 &     0.00 &     0.00 \\
13 &  0.01 &    0.00 &     0.00 &     0.00 \\
14 &  0.01 &    0.00 &     0.00 &     0.00 \\
15 &  0.01 &    0.00 &     0.00 &     0.00 \\
16 &  0.00 &    0.00 &     0.00 &     0.00 \\
17 &  0.01 &    0.00 &     0.00 &     0.00 \\
18 &  0.01 &    0.00 &     0.00 &     0.00 \\
19 &  0.03 &    0.00 &     0.00 &     0.00 \\
20 &  0.02 &    0.00 &     0.00 &     0.00 \\
21 &  0.01 &    0.00 &     0.00 &     0.00 \\
22 &  0.04 &    0.00 &     0.00 &     0.00 \\
23 &  0.03 &    0.00 &     0.00 &     0.00 \\
24 &  0.03 &    0.00 &     0.00 &     0.00 \\
25 &  0.02 &    0.00 &     0.00 &     0.00 \\
26 &  0.03 &    0.00 &     0.00 &     0.00 \\
27 &  0.04 &    0.00 &     0.00 &     0.00 \\
28 &  0.04 &    0.00 &     0.00 &     0.00 \\
29 &  0.17 &    0.00 &     0.00 &     0.00 \\
30 &  0.06 &    0.00 &     0.00 &     0.00 \\
31 &  0.26 &    0.00 &     0.00 &     0.00 \\
32 &  0.08 &    0.00 &     0.00 &     0.00 \\
33 &  0.06 &    0.00 &     0.00 &     0.00 \\
34 &  0.07 &    0.00 &     0.00 &     0.00 \\
35 &  0.08 &    0.00 &     0.00 &     0.00 \\
36 &  0.11 &    0.00 &     0.00 &     0.00 \\
37 &  0.12 &    0.00 &     0.00 &     0.00 \\
38 &  0.11 &    0.00 &     0.00 &     0.00 \\
39 &  0.12 &    0.00 &     0.00 &     0.00 \\
40 &  0.15 &    0.00 &     0.00 &     0.00 \\
41 &  0.12 &    0.00 &     0.00 &     0.00 \\
42 &  0.15 &    0.00 &     0.00 &     0.00 \\
43 &  0.16 &    0.00 &     0.00 &     0.00 \\
44 &  0.17 &    0.00 &     0.00 &     0.00 \\
45 &  0.18 &    0.00 &     0.00 &     0.00 \\
46 &  0.19 &    0.00 &     0.00 &     0.00 \\
47 &  0.21 &    0.00 &     0.00 &     0.00 \\
48 &  0.15 &    0.00 &     0.00 &     0.00 \\
49 &  0.17 &    0.00 &     0.00 &     0.00 \\
50 &  0.23 &    0.00 &     0.00 &     0.00 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/processed_data/checklist/maximum_resident_ltl.tex <==
\begin{table}
\centering
\caption{checklist, Maximum Resident Size in K to Compute LTL}
\label{checklist_LTL_size}
\begin{tabular}{lllll}
\toprule
{} &    BTC & Leaf\_v2 & Total\_v2 & Total\_v3 \\
\midrule
1  &  16476 &   16642 &    16446 &    16446 \\
2  &  16634 &   17106 &    16598 &    16548 \\
3  &  16978 &   17522 &    16844 &    16748 \\
4  &  17334 &   18192 &    17288 &    16968 \\
5  &  17726 &   18852 &    18940 &    17238 \\
6  &  18350 &   19596 &    25818 &    17456 \\
7  &  18562 &   20440 &    53528 &    17790 \\
8  &  19224 &   21354 &   186336 &    18358 \\
9  &  19784 &   22456 &   697398 &    18752 \\
10 &  20564 &   23484 &        - &    19202 \\
11 &  21338 &   24720 &        - &    19732 \\
12 &  22312 &   26004 &        - &    20382 \\
13 &  23788 &   27418 &        - &    20942 \\
14 &  24810 &   29284 &        - &    21654 \\
15 &  33468 &   30838 &        - &    22438 \\
16 &  33222 &   32602 &        - &    23706 \\
17 &  33380 &   34418 &        - &    24468 \\
18 &  35122 &   36368 &        - &    25368 \\
19 &  37538 &   38178 &        - &    26296 \\
20 &  39548 &   40292 &        - &    27414 \\
21 &  40608 &   43002 &        - &    28516 \\
22 &  43892 &   45212 &        - &    29660 \\
23 &  43894 &   47530 &        - &    30858 \\
24 &  45166 &   50118 &        - &    32394 \\
25 &  45958 &   52758 &        - &    33496 \\
26 &  48368 &   55554 &        - &    34940 \\
27 &  48360 &   58398 &        - &    36364 \\
28 &  45070 &   61242 &        - &    38418 \\
29 &  51100 &   64120 &        - &    39856 \\
30 &  51828 &   67168 &        - &    42218 \\
31 &  52406 &   70152 &        - &    44678 \\
32 &  53210 &   73700 &        - &    48396 \\
33 &  53326 &   77216 &        - &    50308 \\
34 &  53998 &   80558 &        - &    52194 \\
35 &  54392 &   83760 &        - &    54224 \\
36 &  55214 &   87504 &        - &    56386 \\
37 &  56380 &   90892 &        - &    59504 \\
38 &  57482 &   94520 &        - &    61898 \\
39 &  58432 &   98058 &        - &    64320 \\
40 &  59530 &  107432 &        - &    67206 \\
41 &  61378 &  112782 &        - &    69238 \\
42 &  63952 &  111382 &        - &    71730 \\
43 &  65760 &  115372 &        - &    74274 \\
44 &  66478 &  126364 &        - &    77874 \\
45 &  68176 &  128116 &        - &    80526 \\
46 &      - &  135478 &        - &    83796 \\
47 &      - &  137170 &        - &    87262 \\
48 &      - &  145052 &        - &    92086 \\
49 &      - &  146814 &        - &    94252 \\
50 &      - &  151726 &        - &    97090 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/processed_data/checklist/reachable_states.tex <==
\begin{table}
\centering
\caption{checklist, Reachable States}
\label{checklist_reach}
\begin{tabular}{lllll}
\toprule
{} &  BTC & Leaf\_v2 &     Total\_v2 &     Total\_v3 \\
\midrule
1  &    3 &       7 &            2 &            2 \\
2  &    5 &      14 &            4 &            4 \\
3  &    7 &      21 &            8 &            8 \\
4  &    9 &      28 &           16 &           16 \\
5  &   11 &      35 &           32 &           32 \\
6  &   13 &      42 &           64 &           64 \\
7  &   15 &      49 &          128 &          128 \\
8  &   17 &      56 &          256 &          256 \\
9  &   19 &      63 &          512 &          512 \\
10 &   21 &      70 &         1024 &         1024 \\
11 &   23 &      77 &         2048 &         2048 \\
12 &   25 &      84 &         4096 &         4096 \\
13 &   27 &      91 &         8192 &         8192 \\
14 &   29 &      98 &        16384 &        16384 \\
15 &   31 &     105 &        32768 &        32768 \\
16 &   33 &     112 &        65536 &        65536 \\
17 &   35 &     119 &       131072 &       131072 \\
18 &   37 &     126 &       262144 &       262144 \\
19 &   39 &     133 &       524288 &       524288 \\
20 &   41 &     140 &  1.04858e+06 &  1.04858e+06 \\
21 &   43 &     147 &  2.09715e+06 &  2.09715e+06 \\
22 &   45 &     154 &   4.1943e+06 &   4.1943e+06 \\
23 &   47 &     161 &  8.38861e+06 &  8.38861e+06 \\
24 &   49 &     168 &  1.67772e+07 &  1.67772e+07 \\
25 &   51 &     175 &  3.35544e+07 &  3.35544e+07 \\
26 &   53 &     182 &  6.71089e+07 &  6.71089e+07 \\
27 &   55 &     189 &  1.34218e+08 &  1.34218e+08 \\
28 &   57 &     196 &  2.68435e+08 &  2.68435e+08 \\
29 &   59 &     203 &  5.36871e+08 &  5.36871e+08 \\
30 &   61 &     210 &  1.07374e+09 &  1.07374e+09 \\
31 &   63 &     217 &  2.14748e+09 &  2.14748e+09 \\
32 &   65 &     224 &  4.29497e+09 &  4.29497e+09 \\
33 &   67 &     231 &  8.58993e+09 &  8.58993e+09 \\
34 &   69 &     238 &  1.71799e+10 &  1.71799e+10 \\
35 &   71 &     245 &  3.43597e+10 &  3.43597e+10 \\
36 &   73 &     252 &  6.87195e+10 &  6.87195e+10 \\
37 &   75 &     259 &  1.37439e+11 &  1.37439e+11 \\
38 &   77 &     266 &  2.74878e+11 &  2.74878e+11 \\
39 &   79 &     273 &  5.49756e+11 &  5.49756e+11 \\
40 &   81 &     280 &  1.09951e+12 &  1.09951e+12 \\
41 &   83 &     287 &  2.19902e+12 &  2.19902e+12 \\
42 &   85 &     294 &  4.39805e+12 &  4.39805e+12 \\
43 &   87 &     301 &  8.79609e+12 &  8.79609e+12 \\
44 &   89 &     308 &  1.75922e+13 &  1.75922e+13 \\
45 &   91 &     315 &  3.51844e+13 &  3.51844e+13 \\
46 &   93 &     322 &  7.03687e+13 &  7.03687e+13 \\
47 &   95 &     329 &  1.40737e+14 &  1.40737e+14 \\
48 &   97 &     336 &  2.81475e+14 &  2.81475e+14 \\
49 &   99 &     343 &   5.6295e+14 &   5.6295e+14 \\
50 &  101 &     350 &   1.1259e+15 &   1.1259e+15 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/processed_data/checklist/total_states.tex <==
\begin{table}
\centering
\caption{checklist, Total States}
\label{checklist_total}
\begin{tabular}{lllll}
\toprule
{} &           BTC & Leaf\_v2 &     Total\_v2 &     Total\_v3 \\
\midrule
1  &            32 &      12 &            2 &            2 \\
2  &          4096 &      36 &            4 &            4 \\
3  &        524288 &      72 &            8 &            8 \\
4  &   6.71089e+07 &     120 &           16 &           16 \\
5  &   8.58993e+09 &     180 &           32 &           32 \\
6  &   1.09951e+12 &     252 &           64 &           64 \\
7  &   1.40737e+14 &     336 &          128 &          128 \\
8  &   1.80144e+16 &     432 &          256 &          256 \\
9  &   2.30584e+18 &     540 &          512 &          512 \\
10 &   2.95148e+20 &     660 &         1024 &         1024 \\
11 &   3.77789e+22 &     792 &         2048 &         2048 \\
12 &    4.8357e+24 &     936 &         4096 &         4096 \\
13 &    6.1897e+26 &    1092 &         8192 &         8192 \\
14 &   7.92282e+28 &    1260 &        16384 &        16384 \\
15 &   1.01412e+31 &    1440 &        32768 &        32768 \\
16 &   1.29807e+33 &    1632 &        65536 &        65536 \\
17 &   1.66153e+35 &    1836 &       131072 &       131072 \\
18 &   2.12676e+37 &    2052 &       262144 &       262144 \\
19 &   2.72226e+39 &    2280 &       524288 &       524288 \\
20 &   3.48449e+41 &    2520 &  1.04858e+06 &  1.04858e+06 \\
21 &   4.46015e+43 &    2772 &  2.09715e+06 &  2.09715e+06 \\
22 &   5.70899e+45 &    3036 &   4.1943e+06 &   4.1943e+06 \\
23 &   7.30751e+47 &    3312 &  8.38861e+06 &  8.38861e+06 \\
24 &   9.35361e+49 &    3600 &  1.67772e+07 &  1.67772e+07 \\
25 &   1.19726e+52 &    3900 &  3.35544e+07 &  3.35544e+07 \\
26 &    1.5325e+54 &    4212 &  6.71089e+07 &  6.71089e+07 \\
27 &   1.96159e+56 &    4536 &  1.34218e+08 &  1.34218e+08 \\
28 &   2.51084e+58 &    4872 &  2.68435e+08 &  2.68435e+08 \\
29 &   3.21388e+60 &    5220 &  5.36871e+08 &  5.36871e+08 \\
30 &   4.11376e+62 &    5580 &  1.07374e+09 &  1.07374e+09 \\
31 &   5.26561e+64 &    5952 &  2.14748e+09 &  2.14748e+09 \\
32 &   6.73999e+66 &    6336 &  4.29497e+09 &  4.29497e+09 \\
33 &   8.62718e+68 &    6732 &  8.58993e+09 &  8.58993e+09 \\
34 &   1.10428e+71 &    7140 &  1.71799e+10 &  1.71799e+10 \\
35 &   1.41348e+73 &    7560 &  3.43597e+10 &  3.43597e+10 \\
36 &   1.80925e+75 &    7992 &  6.87195e+10 &  6.87195e+10 \\
37 &   2.31584e+77 &    8436 &  1.37439e+11 &  1.37439e+11 \\
38 &   2.96428e+79 &    8892 &  2.74878e+11 &  2.74878e+11 \\
39 &   3.79428e+81 &    9360 &  5.49756e+11 &  5.49756e+11 \\
40 &   4.85667e+83 &    9840 &  1.09951e+12 &  1.09951e+12 \\
41 &   6.21654e+85 &   10332 &  2.19902e+12 &  2.19902e+12 \\
42 &   7.95717e+87 &   10836 &  4.39805e+12 &  4.39805e+12 \\
43 &   1.01852e+90 &   11352 &  8.79609e+12 &  8.79609e+12 \\
44 &    1.3037e+92 &   11880 &  1.75922e+13 &  1.75922e+13 \\
45 &   1.66874e+94 &   12420 &  3.51844e+13 &  3.51844e+13 \\
46 &   2.13599e+96 &   12972 &  7.03687e+13 &  7.03687e+13 \\
47 &   2.73406e+98 &   13536 &  1.40737e+14 &  1.40737e+14 \\
48 &   3.4996e+100 &   14112 &  2.81475e+14 &  2.81475e+14 \\
49 &  4.47949e+102 &   14700 &   5.6295e+14 &   5.6295e+14 \\
50 &  5.73375e+104 &   15300 &   1.1259e+15 &   1.1259e+15 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/processed_data/parallel-checklist/diameters.tex <==
\begin{table}
\centering
\caption{parallel-checklist, System Diameter}
\label{parallel-checklist_diam}
\begin{tabular}{lllll}
\toprule
{} &  BTC & Leaf\_v2 & Total\_v2 & Total\_v3 \\
\midrule
1  &    2 &       3 &        1 &        1 \\
2  &    5 &       4 &        1 &        1 \\
3  &    7 &       5 &        1 &        1 \\
4  &    9 &       6 &        1 &        1 \\
5  &   11 &       7 &        1 &        1 \\
6  &   13 &       8 &        1 &        1 \\
7  &   15 &       9 &        1 &        1 \\
8  &   17 &      10 &        1 &        1 \\
9  &   19 &      11 &        1 &        1 \\
10 &   21 &      12 &        1 &        1 \\
11 &   23 &      13 &        1 &        1 \\
12 &   25 &      14 &        1 &        1 \\
13 &   27 &      15 &        1 &        1 \\
14 &   29 &      16 &        1 &        1 \\
15 &   31 &      17 &        1 &        1 \\
16 &   33 &      18 &        1 &        1 \\
17 &   35 &      19 &        1 &        1 \\
18 &   37 &      20 &        1 &        1 \\
19 &   39 &      21 &        1 &        1 \\
20 &   41 &      22 &        1 &        1 \\
21 &   43 &      23 &        1 &        1 \\
22 &   45 &      24 &        1 &        1 \\
23 &   47 &      25 &        1 &        1 \\
24 &   49 &      26 &        1 &        1 \\
25 &   51 &      27 &        1 &        1 \\
26 &   53 &      28 &        1 &        1 \\
27 &   55 &      29 &        1 &        1 \\
28 &   57 &      30 &        1 &        1 \\
29 &   59 &      31 &        1 &        1 \\
30 &   61 &      32 &        1 &        1 \\
31 &   63 &      33 &        1 &        1 \\
32 &   65 &      34 &        1 &        1 \\
33 &   67 &      35 &        1 &        1 \\
34 &   69 &      36 &        1 &        1 \\
35 &   71 &      37 &        1 &        1 \\
36 &   73 &      38 &        1 &        1 \\
37 &   75 &      39 &        1 &        1 \\
38 &   77 &      40 &        1 &        1 \\
39 &   79 &      41 &        1 &        1 \\
40 &   81 &      42 &        1 &        1 \\
41 &   83 &      43 &        1 &        1 \\
42 &   85 &      44 &        1 &        1 \\
43 &   87 &      45 &        1 &        1 \\
44 &   89 &      46 &        1 &        1 \\
45 &   91 &      47 &        1 &        1 \\
46 &   93 &      48 &        1 &        1 \\
47 &   95 &      49 &        1 &        1 \\
48 &   97 &      50 &        1 &        1 \\
49 &   99 &      51 &        1 &        1 \\
50 &  101 &      52 &        1 &        1 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/processed_data/parallel-checklist/elapsed_ltl.tex <==
\begin{table}
\centering
\caption{parallel-checklist, Time in Seconds to Compute LTL}
\label{parallel-checklist_LTL_time}
\begin{tabular}{lllll}
\toprule
{} &     BTC & Leaf\_v2 & Total\_v2 & Total\_v3 \\
\midrule
1  &    0.00 &    0.00 &     0.00 &     0.00 \\
2  &    0.00 &    0.01 &     0.00 &     0.00 \\
3  &    0.01 &    0.02 &     0.00 &     0.00 \\
4  &    0.04 &    0.04 &     0.01 &     0.01 \\
5  &    0.05 &    0.06 &     0.01 &     0.01 \\
6  &    0.11 &    0.10 &     0.01 &     0.02 \\
7  &    0.17 &    0.15 &     0.02 &     0.03 \\
8  &    0.31 &    0.21 &     0.03 &     0.03 \\
9  &    1.88 &    0.29 &     0.03 &     0.04 \\
10 &    1.20 &    0.40 &     0.04 &     0.03 \\
11 &    1.63 &    0.50 &     0.05 &     0.06 \\
12 &    2.54 &    0.63 &     0.06 &     0.06 \\
13 &   58.20 &    0.80 &     0.07 &     0.07 \\
14 &   57.48 &    0.99 &     0.08 &     0.08 \\
15 &   49.61 &    1.20 &     0.08 &     0.10 \\
16 &   96.97 &    1.45 &     0.10 &     0.12 \\
17 &       - &    1.91 &     0.12 &     0.13 \\
18 &  156.54 &    2.05 &     0.12 &     0.13 \\
19 &  242.22 &    2.42 &     0.15 &     0.17 \\
20 &  285.01 &    2.77 &     0.17 &     0.19 \\
21 &       - &    3.18 &     0.19 &     0.20 \\
22 &       - &    3.44 &     0.19 &     0.23 \\
23 &       - &    3.91 &     0.22 &     0.24 \\
24 &       - &    4.50 &     0.24 &     0.27 \\
25 &       - &    5.19 &     0.25 &     0.29 \\
26 &       - &    5.81 &     0.31 &     0.31 \\
27 &       - &    6.37 &     0.29 &     0.40 \\
28 &       - &    7.52 &     0.34 &     0.38 \\
29 &       - &    8.14 &     0.34 &     0.41 \\
30 &       - &    8.93 &     0.40 &     0.48 \\
31 &       - &    9.68 &     0.40 &     0.44 \\
32 &       - &   10.83 &     0.41 &     0.51 \\
33 &       - &   11.67 &     0.47 &     0.53 \\
34 &       - &   12.54 &     0.51 &     0.55 \\
35 &       - &   14.16 &     0.54 &     0.58 \\
36 &       - &   14.97 &     0.60 &     0.71 \\
37 &       - &   16.38 &     0.67 &     0.70 \\
38 &       - &   17.44 &     0.61 &     0.71 \\
39 &       - &   20.48 &     0.68 &     0.73 \\
40 &       - &   22.74 &     0.74 &     0.74 \\
41 &       - &   24.09 &     0.73 &     0.76 \\
42 &       - &   26.54 &     0.76 &     0.81 \\
43 &       - &   27.26 &     0.81 &     0.87 \\
44 &       - &   30.02 &     0.87 &     0.91 \\
45 &       - &   31.90 &     0.83 &     0.95 \\
46 &       - &   34.65 &     0.82 &     0.98 \\
47 &       - &   34.90 &     0.93 &     1.06 \\
48 &       - &   36.57 &     0.95 &     1.09 \\
49 &       - &   38.59 &     0.96 &     1.14 \\
50 &       - &   42.01 &     1.04 &     1.19 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/processed_data/parallel-checklist/elapsed_model.tex <==
\begin{table}
\centering
\caption{parallel-checklist, Time in Seconds to Build Model}
\label{parallel-checklist_model_time}
\begin{tabular}{lllll}
\toprule
{} &   BTC & Leaf\_v2 & Total\_v2 & Total\_v3 \\
\midrule
1  &  0.00 &    0.00 &     0.00 &     0.00 \\
2  &  0.00 &    0.00 &     0.00 &     0.00 \\
3  &  0.00 &    0.00 &     0.00 &     0.00 \\
4  &  0.00 &    0.00 &     0.00 &     0.00 \\
5  &  0.00 &    0.00 &     0.00 &     0.00 \\
6  &  0.00 &    0.01 &     0.00 &     0.00 \\
7  &  0.01 &    0.01 &     0.00 &     0.00 \\
8  &  0.01 &    0.01 &     0.00 &     0.00 \\
9  &  0.00 &    0.01 &     0.00 &     0.00 \\
10 &  0.01 &    0.01 &     0.00 &     0.00 \\
11 &  0.01 &    0.01 &     0.00 &     0.00 \\
12 &  0.01 &    0.01 &     0.00 &     0.00 \\
13 &  0.02 &    0.02 &     0.00 &     0.00 \\
14 &  0.02 &    0.02 &     0.00 &     0.00 \\
15 &  0.03 &    0.02 &     0.00 &     0.00 \\
16 &  0.03 &    0.02 &     0.00 &     0.00 \\
17 &  0.04 &    0.03 &     0.00 &     0.00 \\
18 &  0.04 &    0.03 &     0.00 &     0.01 \\
19 &  0.04 &    0.03 &     0.00 &     0.00 \\
20 &  0.05 &    0.03 &     0.00 &     0.00 \\
21 &  0.05 &    0.04 &     0.00 &     0.00 \\
22 &  0.05 &    0.03 &     0.00 &     0.01 \\
23 &  0.07 &    0.03 &     0.00 &     0.00 \\
24 &  0.09 &    0.04 &     0.00 &     0.00 \\
25 &  0.22 &    0.03 &     0.00 &     0.00 \\
26 &  0.10 &    0.04 &     0.00 &     0.01 \\
27 &  0.10 &    0.04 &     0.01 &     0.01 \\
28 &  0.16 &    0.05 &     0.00 &     0.01 \\
29 &  0.31 &    0.05 &     0.00 &     0.01 \\
30 &  0.18 &    0.05 &     0.00 &     0.00 \\
31 &  0.35 &    0.05 &     0.00 &     0.00 \\
32 &  0.58 &    0.06 &     0.01 &     0.01 \\
33 &  0.85 &    0.05 &     0.00 &     0.01 \\
34 &  0.60 &    0.06 &     0.01 &     0.01 \\
35 &  0.65 &    0.06 &     0.00 &     0.01 \\
36 &  0.65 &    0.06 &     0.01 &     0.01 \\
37 &  0.68 &    0.07 &     0.01 &     0.01 \\
38 &  0.70 &    0.07 &     0.01 &     0.01 \\
39 &  0.79 &    0.07 &     0.01 &     0.00 \\
40 &  0.81 &    0.07 &     0.01 &     0.01 \\
41 &  0.99 &    0.09 &     0.01 &     0.01 \\
42 &  0.90 &    0.07 &     0.01 &     0.01 \\
43 &  0.95 &    0.08 &     0.01 &     0.01 \\
44 &  1.01 &    0.09 &     0.01 &     0.01 \\
45 &  1.14 &    0.09 &     0.01 &     0.01 \\
46 &  1.10 &    0.08 &     0.01 &     0.01 \\
47 &  1.22 &    0.09 &     0.01 &     0.01 \\
48 &  1.46 &    0.09 &     0.01 &     0.01 \\
49 &  3.75 &    0.09 &     0.01 &     0.01 \\
50 &  1.49 &    0.09 &     0.01 &     0.01 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/processed_data/parallel-checklist/elapsed_states.tex <==
\begin{table}
\centering
\caption{parallel-checklist, Time in Seconds to Compute Reachability}
\label{parallel-checklist_states_time}
\begin{tabular}{lllll}
\toprule
{} &   BTC & Leaf\_v2 & Total\_v2 & Total\_v3 \\
\midrule
1  &  0.00 &    0.00 &     0.00 &     0.00 \\
2  &  0.00 &    0.00 &     0.00 &     0.00 \\
3  &  0.00 &    0.00 &     0.00 &     0.00 \\
4  &  0.00 &    0.00 &     0.00 &     0.00 \\
5  &  0.00 &    0.00 &     0.00 &     0.00 \\
6  &  0.00 &    0.00 &     0.00 &     0.00 \\
7  &  0.00 &    0.00 &     0.00 &     0.00 \\
8  &  0.00 &    0.00 &     0.00 &     0.00 \\
9  &  0.01 &    0.00 &     0.00 &     0.00 \\
10 &  0.01 &    0.00 &     0.00 &     0.00 \\
11 &  0.00 &    0.00 &     0.00 &     0.00 \\
12 &  0.02 &    0.00 &     0.00 &     0.00 \\
13 &  0.01 &    0.00 &     0.00 &     0.00 \\
14 &  0.01 &    0.00 &     0.00 &     0.00 \\
15 &  0.02 &    0.00 &     0.00 &     0.00 \\
16 &  0.02 &    0.00 &     0.00 &     0.00 \\
17 &  0.03 &    0.00 &     0.00 &     0.00 \\
18 &  0.03 &    0.00 &     0.00 &     0.00 \\
19 &  0.03 &    0.00 &     0.00 &     0.00 \\
20 &  0.04 &    0.00 &     0.00 &     0.00 \\
21 &  0.04 &    0.00 &     0.00 &     0.00 \\
22 &  0.04 &    0.00 &     0.00 &     0.00 \\
23 &  0.05 &    0.00 &     0.00 &     0.00 \\
24 &  0.05 &    0.00 &     0.00 &     0.00 \\
25 &  0.11 &    0.00 &     0.00 &     0.00 \\
26 &  0.11 &    0.00 &     0.00 &     0.00 \\
27 &  0.11 &    0.00 &     0.00 &     0.00 \\
28 &  0.10 &    0.00 &     0.00 &     0.00 \\
29 &  0.13 &    0.00 &     0.00 &     0.00 \\
30 &  0.09 &    0.00 &     0.00 &     0.00 \\
31 &  0.13 &    0.00 &     0.00 &     0.00 \\
32 &  0.15 &    0.00 &     0.00 &     0.00 \\
33 &  0.17 &    0.00 &     0.00 &     0.00 \\
34 &  0.18 &    0.00 &     0.00 &     0.00 \\
35 &  0.16 &    0.00 &     0.00 &     0.00 \\
36 &  0.19 &    0.00 &     0.00 &     0.00 \\
37 &  0.22 &    0.00 &     0.00 &     0.00 \\
38 &  0.19 &    0.00 &     0.00 &     0.00 \\
39 &  0.23 &    0.00 &     0.00 &     0.00 \\
40 &  0.25 &    0.00 &     0.00 &     0.00 \\
41 &  0.28 &    0.00 &     0.00 &     0.00 \\
42 &  0.28 &    0.00 &     0.00 &     0.00 \\
43 &  0.30 &    0.00 &     0.00 &     0.00 \\
44 &  0.30 &    0.00 &     0.00 &     0.00 \\
45 &  0.37 &    0.00 &     0.00 &     0.00 \\
46 &  0.31 &    0.00 &     0.00 &     0.00 \\
47 &  0.37 &    0.00 &     0.00 &     0.00 \\
48 &  0.41 &    0.00 &     0.00 &     0.00 \\
49 &  0.48 &    0.00 &     0.00 &     0.00 \\
50 &  0.52 &    0.00 &     0.00 &     0.00 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/processed_data/parallel-checklist/maximum_resident_ltl.tex <==
\begin{table}
\centering
\caption{parallel-checklist, Maximum Resident Size in K to Compute LTL}
\label{parallel-checklist_LTL_size}
\begin{tabular}{lllll}
\toprule
{} &    BTC & Leaf\_v2 & Total\_v2 & Total\_v3 \\
\midrule
1  &  16476 &   16644 &    16446 &    16446 \\
2  &  16766 &   16974 &    16548 &    16548 \\
3  &  17170 &   17632 &    16690 &    16694 \\
4  &  17810 &   18188 &    16834 &    16890 \\
5  &  18334 &   18998 &    17020 &    17030 \\
6  &  18802 &   19748 &    17194 &    17218 \\
7  &  20364 &   20610 &    17400 &    17438 \\
8  &  21450 &   21728 &    17740 &    17778 \\
9  &  23300 &   22910 &    17974 &    17984 \\
10 &  24516 &   24102 &    18186 &    18356 \\
11 &  27452 &   25578 &    18512 &    18668 \\
12 &  27484 &   27066 &    18932 &    19048 \\
13 &  44366 &   28564 &    19162 &    19434 \\
14 &  41196 &   30284 &    19594 &    19726 \\
15 &  41450 &   32040 &    20028 &    20202 \\
16 &  42448 &   34110 &    20382 &    20596 \\
17 &      - &   36304 &    20856 &    21126 \\
18 &  42738 &   39046 &    21304 &    21570 \\
19 &  44206 &   41412 &    21764 &    22158 \\
20 &  44096 &   43974 &    22280 &    22640 \\
21 &      - &   46842 &    22870 &    23242 \\
22 &      - &   49320 &    23322 &    23802 \\
23 &      - &   52856 &    23888 &    24402 \\
24 &      - &   56802 &    24570 &    24970 \\
25 &      - &   60062 &    25066 &    25682 \\
26 &      - &   62722 &    25734 &    26406 \\
27 &      - &   66112 &    26350 &    27144 \\
28 &      - &   70862 &    27072 &    27830 \\
29 &      - &   74524 &    27714 &    28548 \\
30 &      - &   78646 &    28390 &    29310 \\
31 &      - &   81686 &    29220 &    30024 \\
32 &      - &   91356 &    29936 &    30838 \\
33 &      - &   96632 &    30678 &    32540 \\
34 &      - &  101670 &    31460 &    33534 \\
35 &      - &  106294 &    32236 &    34416 \\
36 &      - &  111524 &    33142 &    35266 \\
37 &      - &  117050 &    34884 &    36544 \\
38 &      - &  122354 &    35782 &    37512 \\
39 &      - &  127300 &    36888 &    38502 \\
40 &      - &  132464 &    38084 &    39548 \\
41 &      - &  138686 &    38968 &    40582 \\
42 &      - &  146100 &    40008 &    41658 \\
43 &      - &  149144 &    41000 &    42722 \\
44 &      - &  157934 &    42024 &    43838 \\
45 &      - &  166110 &    42996 &    44976 \\
46 &      - &  171752 &    44150 &    46186 \\
47 &      - &  180714 &    45230 &    47316 \\
48 &      - &  187310 &    46458 &    48500 \\
49 &      - &  194996 &    47598 &    49776 \\
50 &      - &  201464 &    48718 &    50988 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/processed_data/parallel-checklist/reachable_states.tex <==
\begin{table}
\centering
\caption{parallel-checklist, Reachable States}
\label{parallel-checklist_reach}
\begin{tabular}{lllll}
\toprule
{} &  BTC & Leaf\_v2 &     Total\_v2 &     Total\_v3 \\
\midrule
1  &    3 &       7 &            2 &            2 \\
2  &    8 &      19 &            4 &            4 \\
3  &   12 &      43 &            8 &            8 \\
4  &   16 &      55 &           16 &           16 \\
5  &   20 &     103 &           32 &           32 \\
6  &   24 &     127 &           64 &           64 \\
7  &   28 &     151 &          128 &          128 \\
8  &   32 &     163 &          256 &          256 \\
9  &   36 &     259 &          512 &          512 \\
10 &   40 &     307 &         1024 &         1024 \\
11 &   44 &     355 &         2048 &         2048 \\
12 &   48 &     379 &         4096 &         4096 \\
13 &   52 &     427 &         8192 &         8192 \\
14 &   56 &     451 &        16384 &        16384 \\
15 &   60 &     475 &        32768 &        32768 \\
16 &   64 &     487 &        65536 &        65536 \\
17 &   68 &     679 &       131072 &       131072 \\
18 &   72 &     775 &       262144 &       262144 \\
19 &   76 &     871 &       524288 &       524288 \\
20 &   80 &     919 &  1.04858e+06 &  1.04858e+06 \\
21 &   84 &    1015 &  2.09715e+06 &  2.09715e+06 \\
22 &   88 &    1063 &   4.1943e+06 &   4.1943e+06 \\
23 &   92 &    1111 &  8.38861e+06 &  8.38861e+06 \\
24 &   96 &    1135 &  1.67772e+07 &  1.67772e+07 \\
25 &  100 &    1231 &  3.35544e+07 &  3.35544e+07 \\
26 &  104 &    1279 &  6.71089e+07 &  6.71089e+07 \\
27 &  108 &    1327 &  1.34218e+08 &  1.34218e+08 \\
28 &  112 &    1351 &  2.68435e+08 &  2.68435e+08 \\
29 &  116 &    1399 &  5.36871e+08 &  5.36871e+08 \\
30 &  120 &    1423 &  1.07374e+09 &  1.07374e+09 \\
31 &  124 &    1447 &  2.14748e+09 &  2.14748e+09 \\
32 &  128 &    1459 &  4.29497e+09 &  4.29497e+09 \\
33 &  132 &    1843 &  8.58993e+09 &  8.58993e+09 \\
34 &  136 &    2035 &  1.71799e+10 &  1.71799e+10 \\
35 &  140 &    2227 &  3.43597e+10 &  3.43597e+10 \\
36 &  144 &    2323 &  6.87195e+10 &  6.87195e+10 \\
37 &  148 &    2515 &  1.37439e+11 &  1.37439e+11 \\
38 &  152 &    2611 &  2.74878e+11 &  2.74878e+11 \\
39 &  156 &    2707 &  5.49756e+11 &  5.49756e+11 \\
40 &  160 &    2755 &  1.09951e+12 &  1.09951e+12 \\
41 &  164 &    2947 &  2.19902e+12 &  2.19902e+12 \\
42 &  168 &    3043 &  4.39805e+12 &  4.39805e+12 \\
43 &  172 &    3139 &  8.79609e+12 &  8.79609e+12 \\
44 &  176 &    3187 &  1.75922e+13 &  1.75922e+13 \\
45 &  180 &    3283 &  3.51844e+13 &  3.51844e+13 \\
46 &  184 &    3331 &  7.03687e+13 &  7.03687e+13 \\
47 &  188 &    3379 &  1.40737e+14 &  1.40737e+14 \\
48 &  192 &    3403 &  2.81475e+14 &  2.81475e+14 \\
49 &  196 &    3595 &   5.6295e+14 &   5.6295e+14 \\
50 &  200 &    3691 &   1.1259e+15 &   1.1259e+15 \\
\bottomrule
\end{tabular}
\end{table}


==> Tables/processed_data/parallel-checklist/total_states.tex <==
\begin{table}
\centering
\caption{parallel-checklist, Total States}
\label{parallel-checklist_total}
\begin{tabular}{lllll}
\toprule
{} &           BTC &      Leaf\_v2 &     Total\_v2 &     Total\_v3 \\
\midrule
1  &            32 &           12 &            2 &            2 \\
2  &          8192 &           54 &            4 &            4 \\
3  &   2.09715e+06 &          216 &            8 &            8 \\
4  &   5.36871e+08 &          810 &           16 &           16 \\
5  &   1.37439e+11 &         2916 &           32 &           32 \\
6  &   3.51844e+13 &        10206 &           64 &           64 \\
7  &    9.0072e+15 &        34992 &          128 &          128 \\
8  &   2.30584e+18 &       118098 &          256 &          256 \\
9  &   5.90296e+20 &       393660 &          512 &          512 \\
10 &   1.51116e+23 &  1.29908e+06 &         1024 &         1024 \\
11 &   3.86856e+25 &  4.25153e+06 &         2048 &         2048 \\
12 &   9.90352e+27 &  1.38175e+07 &         4096 &         4096 \\
13 &    2.5353e+30 &   4.4641e+07 &         8192 &         8192 \\
14 &   6.49037e+32 &  1.43489e+08 &        16384 &        16384 \\
15 &   1.66153e+35 &  4.59165e+08 &        32768 &        32768 \\
16 &   4.25353e+37 &  1.46359e+09 &        65536 &        65536 \\
17 &    1.0889e+40 &  4.64905e+09 &       131072 &       131072 \\
18 &   2.78759e+42 &   1.4722e+10 &       262144 &       262144 \\
19 &   7.13624e+44 &  4.64905e+10 &       524288 &       524288 \\
20 &   1.82688e+47 &  1.46445e+11 &  1.04858e+06 &  1.04858e+06 \\
21 &   4.67681e+49 &  4.60256e+11 &  2.09715e+06 &  2.09715e+06 \\
22 &   1.19726e+52 &  1.44353e+12 &   4.1943e+06 &   4.1943e+06 \\
23 &   3.06499e+54 &  4.51887e+12 &  8.38861e+06 &  8.38861e+06 \\
24 &   7.84638e+56 &  1.41215e+13 &  1.67772e+07 &  1.67772e+07 \\
25 &   2.00867e+59 &   4.4059e+13 &  3.35544e+07 &  3.35544e+07 \\
26 &    5.1422e+61 &  1.37261e+14 &  6.71089e+07 &  6.71089e+07 \\
27 &    1.3164e+64 &  4.27033e+14 &  1.34218e+08 &  1.34218e+08 \\
28 &   3.36999e+66 &  1.32685e+15 &  2.68435e+08 &  2.68435e+08 \\
29 &   8.62718e+68 &  4.11782e+15 &  5.36871e+08 &  5.36871e+08 \\
30 &   2.20856e+71 &  1.27653e+16 &  1.07374e+09 &  1.07374e+09 \\
31 &   5.65391e+73 &  3.95311e+16 &  2.14748e+09 &  2.14748e+09 \\
32 &    1.4474e+76 &  1.22299e+17 &  4.29497e+09 &  4.29497e+09 \\
33 &   3.70535e+78 &  3.78016e+17 &  8.58993e+09 &  8.58993e+09 \\
34 &   9.48569e+80 &   1.1674e+18 &  1.71799e+10 &  1.71799e+10 \\
35 &   2.42834e+83 &  3.60227e+18 &  3.43597e+10 &  3.43597e+10 \\
36 &   6.21654e+85 &   1.1107e+19 &  6.87195e+10 &  6.87195e+10 \\
37 &   1.59143e+88 &  3.42216e+19 &  1.37439e+11 &  1.37439e+11 \\
38 &   4.07407e+90 &  1.05366e+20 &  2.74878e+11 &  2.74878e+11 \\
39 &   1.04296e+93 &  3.24204e+20 &  5.49756e+11 &  5.49756e+11 \\
40 &   2.66998e+95 &  9.96929e+20 &  1.09951e+12 &  1.09951e+12 \\
41 &   6.83516e+97 &  3.06373e+21 &  2.19902e+12 &  2.19902e+12 \\
42 &   1.7498e+100 &  9.41003e+21 &  4.39805e+12 &  4.39805e+12 \\
43 &  4.47949e+102 &  2.88866e+22 &  8.79609e+12 &  8.79609e+12 \\
44 &  1.14675e+105 &  8.86294e+22 &  1.75922e+13 &  1.75922e+13 \\
45 &  2.93568e+107 &  2.71797e+23 &  3.51844e+13 &  3.51844e+13 \\
46 &  7.51534e+109 &  8.33116e+23 &  7.03687e+13 &  7.03687e+13 \\
47 &  1.92393e+112 &  2.55253e+24 &  1.40737e+14 &  1.40737e+14 \\
48 &  4.92525e+114 &  7.81711e+24 &  2.81475e+14 &  2.81475e+14 \\
49 &  1.26086e+117 &  2.39299e+25 &   5.6295e+14 &   5.6295e+14 \\
50 &  3.22781e+119 &  7.32256e+25 &   1.1259e+15 &   1.1259e+15 \\
\bottomrule
\end{tabular}
\end{table}


==> Utility/Un_Macros.tex <==
%-------------------------------------------------------------
%----------Admin. Admin stuff should only be set if this is being compiled solo. If not solo, default to global.
%-------------------------------------------------------------


%----------notes
\ifnum\DocumentIdentifier=\PaperTwentyTwoSEFM{}
\let \todo \undefined{}
\let \TODO \undefined{}
\else{}
\fi{}


%----------citations
\ifnum\DocumentIdentifier=\PaperTwentyTwoSEFM{}
\let \CiteAsText \undefined{}
\let \CiteAsRef \undefined{}
\else{}
\fi{}


%----------environments
\ifnum\DocumentIdentifier=\PaperTwentyTwoSEFM{}
%\let definition \undefined{}
\else{}
\fi{}


%------IsX section
\let \IsDecorator \undefined{}
\let \IsParallel \undefined{}
\let \IsParallelSynch \undefined{}
\let \IsParallelUnsynch \undefined{}
\let \IsRoot \undefined{}
\let \IsSelector \undefined{}
\let \IsSelectorWithMemory \undefined{}
\let \IsSequence \undefined{}
\let \IsSequenceWithMemory \undefined{}
\let \IsSkipped \undefined{}
\let \IsLeaf \undefined{}

%---------------related nodes
\let \LastChild \undefined{}
\let \FirstChild \undefined{}
\let \Parent \undefined{}
\let \LNeigh \undefined{}
\let \RNeigh \undefined{}
\let \Child \undefined{}

%-----------misc
\let \ActiveNode \undefined{}
\let \Active \undefined{}
\let \Status \undefined{}
\let \NextNode \undefined{}
\let \NextNonSkippedChild \undefined{}
\let \ResumeFrom \undefined{}
\let \PriorSuccess \undefined{}
\let \PriorFailure \undefined{}
\let \SkipChild \undefined{}

% %----------Tree Sets
\let \Children \undefined{}
\let \Ancestors \undefined{}

% % -----------Status section
\let \ParallelStatus \undefined{}
\let \FoundFailure \undefined{}
\let \SuccessCount \undefined{}
\let \RunningCount \undefined{}
\let \SuccessThreshold \undefined{}
\let \SelectorStatus \undefined{}
\let \SequenceStatus \undefined{}
\let \LeafStatus \undefined{}
\let \DecoratorStatus \undefined{}

% %----------constants
\let \Invalid \undefined{}
\let \Failure \undefined{}
\let \Running \undefined{}
\let \Success \undefined{}
\let \RootNode \undefined{}
